Instance-guided Cartoon Editing with a Large-scale Dataset

Cartoon editing, appreciated by both professional illustrators and hobbyists, allows extensive creative freedom and the development of original narratives within the cartoon domain. However, the existing literature on cartoon editing is complex and leans heavily on manual operations, owing to the challenge of automatic identification of individual character instances. Therefore, an automated segmentation of these elements becomes imperative to facilitate a variety of cartoon editing applications such as visual style editing, motion decomposition and transfer, and the computation of stereoscopic depths for an enriched visual experience. Unfortunately, most current segmentation methods are designed for natural photographs, failing to recognize from the intricate aesthetics of cartoon subjects, thus lowering segmentation quality. The major challenge stems from two key shortcomings: the rarity of high-quality cartoon dedicated datasets and the absence of competent models for high-resolution instance extraction on cartoons. To address this, we introduce a high-quality dataset of over 100k paired high-resolution cartoon images and their instance labeling masks. We also present an instance-aware image segmentation model that can generate accurate, high-resolution segmentation masks for characters in cartoon images. We present that the proposed approach enables a range of segmentation-dependent cartoon editing applications like 3D Ken Burns parallax effects, text-guided cartoon style editing, and puppet animation from illustrations and manga.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> includes/application_old.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/3dkenburns.pdf}
    \caption{3D Ken Burns guided by instance masks. (a) Input cartoon image. The orange and magenta boxes indicates the camera views at clip beginning and end, respectively. (b) Depth map predicted with the guidance of our generated instance masks. (c) Naive novel view synthesis inevitably produces visual gaps (e.g., black pixels). (d) The instance masks helps perform visually pleasant inpainting of the background for seamless novel view synthesis. (e) Without guidance of instance masks, existing 3D Ken Burns method~\cite{3dkenburns} may lead to false geometry estimation and blurry artifacts at the occluded areas. (f) With instance guidance, our method generates visually pleasant novel views at all frames.}
    \label{fig:3dkenburns}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/style_editing.pdf}
    \caption{Instance-aware style editing with global prompt \textit{holliemengert artstyle} (top), \textit{artist\_cg} (bottom). In absence of instance guidance, the diffusion-based style editing does not maintain the context of the subjects, resulting in visual inconsistency across each subject. Conversely, our approach successfully transfers the style while preserving the visual semantics simultaneously.}
    \label{fig:style_editing}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/puppet_animation.pdf}
    \caption{Motion manga generation based on a single manga image and the instance masks predicted by our cartoon segmentation method.}
    \label{fig:motion_manga}
\end{figure*}

The high-quality instance-level extraction of cartoon subjects enables various cartoon editing applications. These were previously considered challenging and time-consuming due to the significant reliance on manual segmentation of scenes and characters. In this section, we introduce three major applications essential to the real-world production of animations, comics, and manga. These include 3D Ken Burns, Cartoon Style Editing, and Motion Manga.

\subsection{3D Ken Burns}
An innovative use of our proposed instance-aware cartoon and animation parsing approach lies in the 3D Ken Burns effect \cite{3dkenburns}. This effect simulates the parallax visual experience on a single static cartoon or manga frame, enhancing the visual richness and immersion of 2D artworks. To create the 3D Ken Burns effect, depth information is needed to guide the rendering of frames for a specified camera movement. For each rendered frame, inpainting of the background is necessary to produce hole-free frames. However, in the absence of instance mask guidance, neither depth estimation nor inpainting proves to be a simple task. Hence, the existing 3D Ken Burns method typically struggles to generate frames free of artifacts (Fig.~\ref{fig:3dkenburns} (e)).

We leverage the instance masks in depth estimation by requiring the pixels inside the same instance to have the same depth value. We utilize the methodology delineated in~\cite{yin2022towards} to compute a depth map for the input cartoon image, since this method yields more consistent and smoother depth estimations, exhibiting reduced noise and fewer singularities in the resulting depth image (Fig.~\ref{fig:3dkenburns} (b)). However, since this method is proposed for natural photographs without instance awareness, so the generated depth map usually fails to recognize the depth difference between different subjects or between subjects and background in 2D cartoons. Therefore, we further propose to optimize the depth for 2D cartoon images by applying an average pooling filter on the depth of each subject instance. The final depth map presents clear depth difference between different subjects and between subjects and background, as shown in Fig.~\ref{fig:3dkenburns} (c).
The depth map enables the rendering of the scene at an arbitrary camera's angle by reconstructing the point cloud structure and reshading with texture information from the raster pixel values of the original image, as outlined in~\cite{3dkenburns}. For generating 3D Ken Burns effect, a movement path of the camera can be set, such as linearly panning and zooming, and a sequence of frames can be rendered along the camera's movement path. Rendering these novel views is straightforward, but when the camera angles deviate from the original centered positions, there will inevitably be gaps in the rendered frames due to lack of information that does not exist in the original image (Fig.~\ref{fig:3dkenburns} (d)).

Numerous inpainting methods have been proposed, such as PatchMatch~\cite{patchmatch} and latent diffusion~\cite{latentdiffusion}, that can be utilized to inpaint the gaps. Without instance guidance, the gaps are inpainted based on a mixture of foreground and background information, which leads to obvious inpainting artifacts (Fig.~\ref{fig:3dkenburns} (e)), as the gaps are typically background behind foreground subjects. In comparisons, with the extracted instance masks, we are able to inpaint the gaps purely based on background information. We utilize latent diffusion~\cite{latentdiffusion} to synthesize high-quality background images for all frames by masking out the gaps and foreground instances (Fig.~\ref{fig:3dkenburns} (f)). In particular, to avoid creating a new, imagined subject in the masked area during the inpainting while maintaining texture and semantic continuity, we regulate the denoising diffusion in the \emph{text} space using the CLIP encoder. Throughout each diffusion step, we aim to retain CLIP semantics aligned with the pre-inpainting background and penalize semantics that may lead to unintended subjects in the inpainted outputs. To obtain text-based embedding for the background, we initially fill the gaps using PatchMatch with patch size $=3$, and feed this roughly inpainted background into a SwinV2 Tagger~\cite{swinv2tagger} model. This process generates a set of visual tags for the background, which we use as an additional constraint to ensure consistency in visual semantics. Conversely, to avoid unwanted subjects from being synthesized, we define a set of negative prompts~\footnote{The prompt is set to: \textit{human, single, person, girl, 1girl, boy, 1boy, creature, animal, alien, robot, body}} that serve to deter the synthesis of these specific visual semantics. In our experiments, we used the DPM++ 2M Karras scheduler with 32 diffusion steps, and we set the latent diffusion style translation strength as 0.75.  Please refer to the supplemental material for more examples regarding the inpainting algorithm and the prompt design.

This 3D Ken Burns application enables the creation of dynamic, multi-layered scenes from a single static image, reducing the time and effort required in traditional animation production. It may also potentially transform the way we consume and interact with 2D media, paving the way for more engaging, immersive, and visually compelling storytelling in cartoons, animations, and manga.

%Recognizing that the occluded areas are typically background behind foreground subjects, we propose handling the inpainting of these regions. An immediate challenge appears when we find that traditional inpainting methods like PatchMatch~\cite{patchmatch} perform well in extending textures, but may not preserve visual semantics because the algorithm is purely local texture-based. In contrast, the inpainting method in latent diffusion methods~\cite{latentdiffusion} can synthesize high-quality inpainting results for masked areas, but they may be overzealous, recognizing that the masked area actually belongs to a subject instance and creating a new, imagined subject in the masked area. This contradicts our aim of synthesizing a complete, uninterrupted background. To maintain both texture and semantic continuity during inpainting, we regulate the denoising diffusion in the \emph{text} space using the CLIP encoder.  
%level parsing of cartoons and animations, depth information can be automatically acquired to differentiate different elements, such as characters, objects, and background. This enables element-aware inpainting and the creation of dynamic, multi-layered scenes from a single static image, reducing the time and effort required in traditional animation production. Furthermore, this application may potentially transform the way we consume and interact with 2D media, paving the way for more engaging, immersive, and visually compelling storytelling in cartoons, animations, and manga.

%(Still I believe we need a figure, probably will be inside the supplemental.)



% negative prompt for all background: lowres, ((bad anatomy)), ((bad hands)), text, missing finger, extra digits, fewer digits, blurry, ((mutated hands and fingers)), (poorly drawn face), ((mutation)), ((deformed face)), (ugly), ((bad proportions)), ((extra limbs)), extra face, (double head), (extra head), ((extra feet)), monster, logo, cropped, worst quality, low quality, normal quality, jpeg, humpbacked, long body, long neck, ((jpeg artifacts)),((person)), character, 1girl, 1boy

% negative prompt for all subjects: lowres, ((bad anatomy)), ((bad hands)), text, missing finger, extra digits, fewer digits, blurry, ((mutated hands and fingers)), (poorly drawn face), ((mutation)), ((deformed face)), (ugly), ((bad proportions)), ((extra limbs)), extra face, (double head), (extra head), ((extra feet)), monster, logo, cropped, worst quality, low quality, normal quality, jpeg, humpbacked, long body, long neck, ((jpeg artifacts))

% image 1:
% bg prompt: speech_bubble,english_text,tree,no_humans,masterpiece, best quality,

% subject1 prompt: solo,1boy,standing,full_body,masterpiece, best quality

% subject2 prompt: solo,1boy,hat,standing,full_body,male_focus,transparent_background,sandals,masterpiece, best quality

% subject3 prompt: solo,1boy,hat,male_focus,facial_hair,beret,masterpiece, best quality

% subject4 prompt: 1girl,solo,blonde_hair,gloves,dress,jewelry,elbow_gloves,necklace,white_dress,veil,wedding_dress,bridal_veil,masterpiece,best quality


% image 2:
% bg prompt: monochrome,indoors,cup,no_humans,chair,scenery,sepia,brown_theme,masterpiece, best quality, ,holliemengert artstyle

% subject1 prompt: 1girl,solo,short_hair,navel,monochrome,boots,shorts,midriff,masterpiece, best quality,holliemengert artstyle

% subject2 prompt: solo,brown_hair,shirt,1boy,jacket,upper_body,male_focus,necktie,collared_shirt,from_side,black_necktie,masterpiece, best quality, holliemengert artstyle

% subject3 prompt: solo,smile,shirt,1boy,closed_eyes,male_focus,grin,masterpiece, best quality,holliemengert artstyle

% subject4 prompt: solo,1boy,male_focus,facial_hair,beard,bald,masterpiece, best quality,holliemengert artstyle



\subsection{Instance-aware style editing}

The field of image-to-image translation is rapidly progressing, introducing numerous techniques for style conversion across diverse forms of media, including cartoons and anime. While these methods have shown potential in translation between different styles, such as between Japanese anime and western comics or between Shinkai Makoto's movie aesthetics and Studio Ghibli's abstract visual language, they encounter specific hurdles.
Specifically, achieving high-quality translations between arbitrary visual styles requires both a high-level semantic understanding of the visual semantics, as well as the ability to synthesize high-quality textures while maintaining the semantics. Such a requirement is considered effort-intensive and time-consuming, so prior solutions are usually limited to a specific target style, or cannot fully understand the styles of cartoons. Recent diffusion models enabled zero-shot image translation that can synthesize arbitrary visual styles, conditioned by a given text prompt. 
However, without instance-level guidance during image synthesis, these models generally fail to preserve the identity and visual semantics of the instances, as this information is dismissed during the diffusion noise schedule, and not reintroduced during the denoising diffusion steps (Fig.~\ref{fig:style_editing} (b)). What's more, these models also lack precise control over the translation styles for individual subjects, due to the loose instance-wise supervision from the CLIP image encoder. As demonstrated in Fig.~\ref{fig:style_editing} (b), a universal global style target prompt can lead to varied interpretations of visual styles, resulting in an inconsistent overall appearance.

We propose addressing the visual discrepancy problems in cartoons for a consistent style translation by \emph{tightening} the denoising diffusion steps with semantic and visual constraints. This approach maintains an overall uniform look while preserving each individual subject's recognizability. This regularization occurs in two-fold: first, we compute the visual tags for each subject instance and the inpainted background using the SwinV2 tagger~\cite{swinv2tagger}. Subsequently, we feed the computed visual tags together with the target style prompt as a semantic constraint into the img2img denoise diffusion schedule. 
For instance, the text prompt guiding the style translation for the leftmost instance of the top input image in Fig.~\ref{fig:style_editing} combines the computed the instance visual tags \textit{1girl, solo, short\_hair, navel, monochrome, boots, shorts, midriff} and the target style prompt \textit{holliemengert artstyle}. This effectively mitigates issues arose when the CLIP text encoder fails to understand and propagate the target styles to multiple instances in the image. 
Additionally, we employ the lineart ControlNet~\cite{zhang2023adding} as further regularization to ensure the synthesized image retains the same structural lines as the original. This step provides better control over local details, such as hair, hands, and other delicate structures.

In our experiments, all instances receive the same noise seed and schedule for style consistency. We set the img2img strength to 0.75, with a total of 24 denoising steps under the DPM++ 2M Karras denoise scheduler. The ControlNet guidance strength is set to 1. 
Importantly, we find that it is feasible to extend this instance-aware style editing to videos. Our experiments show that our dual CLIP and ControlNet guidance preserves most of the temporal consistency for cartoon videos without requiring any post-processing, such as motion estimation or additional style propagation. Alternatively, we can achieve similar style editing for videos with a lower computational budget by translating the first frame and using EBSynth~\cite{ebsynth} to propagate this style editing throughout the entire cartoon video sequence. Examples of this video-based translation will be illustrated in the supplemental material. 





% \begin{table*}[!t]
% \begin{tabular}{c|ccc|c|ccc}
% \hline
% \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{Our validation dataset}   & \multicolumn{1}{c|}{Manga109} & \multicolumn{3}{c}{Manual segmentation data}                                         \\ \hline
% Method                & Box AP (\%)~$\uparrow$ & Mask AP (\%)~$\uparrow$ & Boundary AP (\%)~$\uparrow$ & Box AP (\%)~$\uparrow$                                      & Box AP (\%)~$\uparrow$ & Mask AP (\%)~$\uparrow$ & Boundary AP (\%)~$\uparrow$ \\ \hline
% Mask-RCNN             &       14.1      &       11.5       &     5.9              &             14.0                                    &               7.8                   &              4.1                     &        0.0          \\
% Grounded SAM          &     77.0        &       68.4       &       42.6           &           25.6                                       &             96.4                     &                    54.4               &           21.1       \\
% YAAS                  &       38.1      &        34.6      &    20.4              &             11.5                                     &                 95.1                 &                  84.6                 &         32.6         \\
% Ours                  &      \textbf{91.1}       &       \textbf{88.0}       &      \textbf{80.1}            &                   \textbf{71.1}                               &                  \textbf{96.5}                &         \textbf{86.5}                          &        \textbf{41.9}          \\ \hline
% \end{tabular}
% \caption{Quantitative comparisons with existing methods.}
% \label{tab:quanlitative_evaluations}
% \end{table*}


\if 0
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/manual_data.pdf}
    \caption{Manually prepared cartoon segmentation ground truth for quantitative evaluations.}
    \label{fig:manual_data}
\end{figure}
\fi

\subsection{Motion Manga}

Motion manga is a type of media that involves imbuing a static manga image with elements of movement and effects. The development of motion manga largely depends on the segmentation of foreground subjects, enabling the independent manipulation of each subject's movement and transformation. Due to the absence of fully automated methods for precise extraction of manga subjects' instance masks, motion manga creation persists as a manual process within the manga industry, proving both time-intensive and labor-expensive. We introduce the first initiative towards a more efficient motion manga creation method, which involves automatic instance mask extraction, background inpainting, and manual definition of movement and transformation for each subject. Leveraging the high-quality instance masks extracted using our model, we can synthesize a high-quality background image, similar to the inpainting approach utilized in 3D Ken Burns effect generation. This synthesized image is then used to create the final motion manga (Fig.~\ref{fig:motion_manga}).

==> includes/dataset_old.tex <==
% Looks like the model is not that important, also we may claim that some future models can make a similar motivation. However, based on our experiments, our current solution can achieve the SOTA performance easily. 

%The lack of a high-quality segmentation solution hinders progress in post-processing techniques for cartoons and manga. 
%Current solutions either struggle with the domain gap due to insufficient high-quality labeled datasets for cartoons, or fail to produce satisfactory segmentations due to their model architecture design.
Due to the large domain gap between natural photographs and cartoons, networks trained with natural photograph dataset generally have unsatisfying performance when applied on cartoons. It is critical to construct a large-scale cartoon dataset featuring instance-level labels for subjects to perform high-quality instance segmentation in cartoons. Ideally, in a supervised setting, human annotators would be invited to label the masks of the instances in each cartoon image. However, due to the time-consuming nature of the task and the challenge of achieving pixel-perfect labeling, it is impractical to obtain a large-scale cartoon segmentation dataset with perfectly labelled masks by manual labeling. 
To create such a large-scale and high-quality cartoon segmentation dataset, we propose a reverse engineering approach that extracts character and object instances from chroma-keying videos and illustrations and simulates the actual composition of cartoons and animations through synthesis. 
%This method addresses these issues while minimizing discrepancies between synthesized images and ground truth to enhance segmentation quality. 
Despite using reverse engineering techniques to create complex datasets is common in the literature, challenges persist in synthesizing ground truths that closely mirror real cartoons. First, the synthesis must cover a wide variety of subjects in cartoons and animations, including diverse characters, poses, and compositions, along with their ground truth labels, and a wide variety of scenic backgrounds. Additionally, the synthesis should produce natural and harmonious compositions akin to actual cartoons.
We present our solutions to these challenges to create a large-scale, high-quality dataset for the subsequent segmentation purposes. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/composition.pdf}
    \caption{Cartoon image synthesis with sampling strategy. Both the foreground instances and the background are from our collected online resources. Speficially, the number of subjects follows a Poisson distribution. We propose two composition schemes chosen randomly, photo-guided subject placement and side-by-side placement. Finally, color harmonization is applied to make the synthesized cartoon image more natural.}
    \label{fig:composition}
\end{figure*}

\subsection{Preparation of foregrounds and backgrounds}

The first step in reverse dataset synthesis involves gathering a diverse set of subject instances and background samples for subsequent composition. Given the fact that manual extraction and labeling are impractical due to resource limitations, we fortuitously discovered that chroma-keying materials from the community provide a rich and natural source of cartoon and animation instances.
As illustrated in Fig.~\ref{fig:chroma_key_videos}, chroma keying materials typically show a moving cartoon character or object on a green or blue background in the format of videos, where the background color is usually denoted as the keying color. A large amount of such chroma-keying materials has been produced from existing cartoon animations by professional artists and amateurs in the animation community to enable the repurposing or extension of cartoon animations with the aid of professional video production software. Given a chroma-keying frame (Fig. \ref{fig:chroma_key} (a)), it is possible to first automatically identify the keying color (Fig. \ref{fig:chroma_key} (b)\&(c)) as alpha channel, and then obtain background-free cartoon characters or objects (Fig. \ref{fig:chroma_key} (d)) and their binary masks in pixels (Fig. \ref{fig:chroma_key} (e)). 

We collect 1,064 chroma-keying videos from popular online anime community sites, such as Niconico, Bilibili, and YouTube. We implement frame skipping at $3$Hz to convert the video into image sequences with reduced pose and appearance similarities. 
With the raw data secured, our next goal is to extract the pixel-level mask for each subject instance from the keying video materials. As these materials generally aim to maximize the differentiation between keying color and foreground color distributions, no fixed color is used as the keying color. In real practice, the keying colors may be green, blue, or any other saturated colors. Therefore, a correct estimation of the keying color is important in extract pixel-level binary masks for the subject instances. 
For each chroma-keying frame, we first apply a bilateral filter \cite{bilateralfilter} with a filter size of 17 and $\sigma=80$ to diminish the potential noise and MPEG artifacts, and at the same time consolidate the variations of the input color distribution. To identify the keying color, we observe that while different chroma-keying videos may use different keying colors, all keying colors are highly saturated and lighted, with both saturation and lightness values above $0.95$ in HSV color space. Besides, the number of keying color pixels is generally dominant in each frame. Based on these observations, we propose to compute the keying color by finding the optimal hue value $H^*$ that produces the maximum pixel count within a local highly saturated and highly lighted range in the HSV color space, i.e.,
\begin{equation}
    \begin{aligned}
    H^* = \underset{H}{\text{argmax}} \ \text{Count}(\text{Range}(H), 
    [0.95, 1],[0.95, 1])
    \end{aligned}
    \label{eqn:foreground_segmentation}
\end{equation}
The function $Count(\cdot,\cdot,\cdot)$ counts the number of pixels whose colors are within the specified HSV range defined by the range of hue (H), the range of saturation (S), and the range of lightness value (V). Especially, the ranges of S and V are fixed to $[0.95, 1]$ since the keying color must be highly saturated and lighted. Since the hue channel is circular, the range of a hue value $Range(H)$ is defined as a circular range of [H-0.025, H+0.025].
\if 0
$$
\text{Range}(x) =
\begin{cases}
  ([x-0.025, x+0.025]) & \text{if } 0.025 \leq x \leq 0.975\\
  ([x+0.975, 1], [0, x+0.025]) & \text{if } 0 \leq x < 0.025 \\
  ([0, x-0.025], [x+0.025, 1]) & \text{if } 0.975 < x \leq 1 \\
\end{cases}
$$
\fi
Fig.~\ref{fig:chroma_key} (b) visualizes the hue distribution computed from the input chroma-keying frame in Fig. \ref{fig:chroma_key} (a). The optimal hue value that produces the maximum pixel count is visualized in Fig. \ref{fig:chroma_key} (c).

To broaden the diversity of the data set, in addition to the subjects based on extracted chroma-keying, we also include the subjects of still illustrations sourced from the Danbooru2021 dataset \cite{danbooru2021}. To ensure that these still illustrations contain only a single subject instance with pixel-perfect labeling, we filtered these illustrations with the \textit{solo} and \textit{transparent\_background} tags such that the alpha channel can be considered as the instance labeling mask. In total, we have collected 65,752 different subjects, among which 26,844 subjects are from the chroma-keying videos and 38,908 subjects are from the still illustrations in Danbooru2021 dataset. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/model.pdf}
    \caption{Overviewing the model architecture, given the cartoon image input, the low-resolution segmentation stage employs backbone and neck networks for multi-scale feature extraction and identifies the bounding boxes and instance-level segmentation masks of subjects. The high-resolution segmentation stage refines each coarse segmentation mask, producing the final high-resolution subject masks. We highlight the supervision objectives in red.}
    \label{fig:model_arch}
\end{figure*}

For background preparation, the quality and variety of the collected background images play a crucial role in the reverse engineering approach. As our subsequent scene composition is intended for segmentation purposes, there is no need to prepare motion-continuous backgrounds.
Thus, we directly collect high-quality still anime backgrounds, which are also referred to as \emph{CG backgrounds} as our background image set. 
Specifically, we have collected 8,163 scenic background samples from the Danbooru2021 dataset by filtering images with the tags \textit{scenery} and \textit{no\_humans}. In addition, we have also collected 8,057 high-quality cartoon background samples from the bizarre pose estimator~\cite{chen2022bizarre}. The resolution of most images (>80\%) in our prepared dataset are above $1024\times768$, ensuring the high-quality requirement for backgrounds is met.

\subsection{Cartoon image synthesis for segmentation}
Having obtained the foreground instances and backgrounds, we proceed with the synthesis of cartoon-like images and segmentation labeling for each instance. It is important to emphasize that the composition of a cartoon image is a nontrivial task, as the positioning of subjects must be appropriate, avoiding both overly sparse and overly crowded placements. Furthermore, to generate sufficient images for effective model training, we need to develop a proper augmentation mechanism.

The synthesis process operates on a fixed target canvas resolution of $720 \times 720$. For each target canvas, we sample a number of subjects $N_{subj}$ based on a Poisson distribution with $\lambda=2.5$ (Fig.~\ref{fig:composition} (a)-(c)) and a random background image (Fig.~\ref{fig:composition} (d)). 
Initially, we apply augmentations to both foreground and background elements to enhance diversity. we adjust the size of the background to the smallest possible dimensions that still cover the target canvas, while keeping its original aspect ratio intact. After that, we perform a random crop on the resized background to fit the canvas (Fig.~\ref{fig:composition} (e)). 
Then, for each foreground instance, we resize the long side of this instance to $[0.15-0.75]\times$ of the canvas side length $720px$. For each resized subject, we continue performing augmentations, including: 
\begin{itemize}
    \item random horizontal flip;
    \item grid distortion, with five grid cells on each side and distort limit set to $(-0.3, 0.3)$; or
    \item random rotation within $\pm30$ degrees. 
\end{itemize}

The computation of the pixel labeling mask for each foreground instance works in the same manner. For the placement of the subject instances for scene composition, we propose two major strategies:

    \paragraph{Photo-guided subject placement} We randomly select a labeled sample from the MSCOCO dataset~\cite{MSCOCO} that contains $>N_{subj}$ \emph{person} instances. We determine the bounding box of each \emph{person} instance in the MSCOCO sample to serve as placement locations, pairing each of our augmented foreground instances with one of these locations. The pairing uses a greedy search to minimize the difference in aspect ratio between the bounding boxes of the placement and the source. This method simulates typical human placement, avoiding excessively crowded foreground compositions. An example is shown in Fig.~\ref{fig:composition} (f).

    \paragraph{Side-by-side placement} The previous approach works well in general cases; however, for cartoon animation frames and illustrations, it is a common technique to render the subjects (especially humans) side-by-side, which looks similarly to group photos for visual impact. To simulate this technique, we establish two parameters, maximum overlap $IoU_{max}=0.8$ and minimum overlap $IoU_{min}=0.15$.  First, we generate a random placement order for the foreground instances and place the first instance with freedom, as long as its bounding box is fully inside the canvas. 
    From the second instance onward, where applicable, we calculate all potential locations where the bounding box of this newly placed instance exhibits IoU values between $IoU_{max}$ and $IoU_{min}$ with the previously placed instance. Specifically, the IoU value is computed as:
    \begin{equation}
        IoU(A, B) = \frac{{|A \cap B|}}{{|A \cup B|}}, 
        \label{eqn:iou}
    \end{equation}
    where $A$ and $B$ are two bounding box locations. 
    We then select a sample from these possible placement locations to finalize the location of the new instance. We continue this process until we have placed the final instance. An example is shown in Fig.~\ref{fig:composition} (g). 
    %For further details on the placement algorithm, please refer to the supplemental material.
    
These two strategies are chosen at random for each target frame. Finally, we conclude the synthesis by enabling post-placement processing to minimize the effect of color discrepancy among the foreground instances and the background. To handle this, we randomly choose one of the following three approaches:

\begin{itemize}
    \item Do nothing; 
    \item Perform a pixel-wise vector quantization using K-means where the number of clusters is randomly selected from $\{12, 16, 32\}$ (Fig.~\ref{fig:composition} (h));
    \item Perform a color histogram matching to align the color distribution for all foreground instances and the background with a randomly selected foreground instance with the approach mentioned in \cite{digitalimageprocessing} (Fig.~\ref{fig:composition} (i)).
\end{itemize}

Finally, we create a new high-quality cartoon segmentation dataset with 107.5k image-mask pairs sourced from 65k foreground instances and 8k background scenic images. Our dataset will be released upon the acceptance of the article.





==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

